Turbulent convection in protoplanetary discs and its role in angular momentum transfer

We present a model for the transport of anisotropic turbulence in an accretion disc. The model uses the Reynolds stress tensor approach in the mean field approximation. To study the role of convection in a protoplanetary disc, we combine the turbulence model with a radiative transfer calculation, and also include convection using the mixing length approximation. We find that the turbulence generated by convection causes the angular momentum of the accretion disc to be directed outwards. We also confirm the conclusions of other authors that turbulent convection is unable to provide the observed disc accretion rates as well as a heat source sufficient for the convection to be self-sustaining. The reasons for the latter are the strong anisotropy of the turbulence together with the low efficiency of the energy transfer from the background velocity shear to the turbulent stress tensor.

==> Makefile <==

SRC := paper
OUT := mnras_v3.4


$(SRC).pdf: $(SRC).tex
	latexmk -pdf $(SRC)


.PHONY: zip
zip:
	zip $(OUT).zip Makefile *.eps *.pdf *.bib *.bbl *.tex *.sty *.cls


.PHONY: clean
clean:
	rm -f *.log *~ \
		$(addprefix $(SRC),.dvi .aux .log .fdb_latexmk .fls .out .toc .cb .cb2)
	rm -f *.log *~ \
		$(addprefix $(SRC),.bbl .blg)

